Towards Inclusive HRI: Using Sim2Real to Address Underrepresentation in Emotion Expression Recognition

Robots and artificial agents that interact with humans should be able to do so without bias and inequity, but facial perception systems have notoriously been found to work more poorly for certain groups of people than others. In our work, we aim to build a system that can perceive humans in a more transparent and inclusive manner. Specifically, we focus on dynamic expressions on the human face, which are difficult to collect for a broad set of people due to privacy concerns and the fact that faces are inherently identifiable. Furthermore, datasets collected from the Internet are not necessarily representative of the general population. We address this problem by offering a Sim2Real approach in which we use a suite of 3D simulated human models that enables us to create an auditable synthetic dataset covering 1) underrepresented facial expressions, outside of the six basic emotions, such as confusion; 2) ethnic or gender minority groups; and 3) a wide range of viewing angles that a robot may encounter a human in the real world. By augmenting a small dynamic emotional expression dataset containing 123 samples with a synthetic dataset containing 4536 samples, we achieved an improvement in accuracy of 15% on our own dataset and 11% on an external benchmark dataset, compared to the performance of the same model architecture without synthetic training data. We also show that this additional step improves accuracy specifically for racial minorities when the architecture's feature extraction weights are trained from scratch.

==> New folder/new.tex <==
. There is no discussion, experiments and comparison between the utilized toolkits/plugins (MakeHuman+FACSHuman) and other widerly used like GANs (StarGAN, StyleGAN, GANimation) or popular 3D Computer Vision techniques. When the authors propose some techniques, it is important to show, prove and persude the viewer why the suggested one is the best one to choose (among others and the sota).

solution:
For example, for the one above we can add a point about why StarGAN etc. is not easily usable (for example, does it generate pose in the way that we need, plus expression, plus lighting?)



concern

I also do not see the reason why the authors have chosen the angry and disgust categories (why they chose confusion is justified). Many existing in-the-wild databases already contain (a lot of images or videos with) these categories, such as Aff-Wild2, DFEW and AffectNet. It would be good if other -non existing in other databases- emotion categories were chosen, as was the case with

A comment on each of these datasets can be added




//////

One of the big concerns was that it was only 3 emotions. But you can argue to first do 1) valence-arousal to narrow down the categories, and  then 2) emotion inference


SOO:
1. focus on valence arousal , maybe emotinet and the circle more
2. instead of emotion recogntion, say facial expression recog or emoton inference


//////////////

CK+: Tell them that this was not in the wild

--
other ones:
DFEW:
AFF-WILD2:
AFFECTNET: IMAGE

==> new.tex <==
. There is no discussion, experiments and comparison between the utilized toolkits/plugins (MakeHuman+FACSHuman) and other widerly used like GANs (StarGAN, StyleGAN, GANimation) or popular 3D Computer Vision techniques. When the authors propose some techniques, it is important to show, prove and persude the viewer why the suggested one is the best one to choose (among others and the sota).

solution:
For example, for the one above we can add a point about why StarGAN etc. is not easily usable (for example, does it generate pose in the way that we need, plus expression, plus lighting?)



concern

I also do not see the reason why the authors have chosen the angry and disgust categories (why they chose confusion is justified). Many existing in-the-wild databases already contain (a lot of images or videos with) these categories, such as Aff-Wild2, DFEW and AffectNet. It would be good if other -non existing in other databases- emotion categories were chosen, as was the case with

A comment on each of these datasets can be added




//////

One of the big concerns was that it was only 3 emotions. But you can argue to first do 1) valence-arousal to narrow down the categories, and  then 2) emotion inference


SOO:
1. focus on valence arousal , maybe emotinet and the circle more
2. instead of emotion recogntion, say facial expression recog or emoton inference


//////////////

CK+: Tell them that this was not in the wild

--
other ones:
DFEW:
AFF-WILD2:
AFFECTNET: IMAGE
